Learning Stochastic Dynamical System via Flow Map Operator

We present a numerical framework for learning unknown stochastic dynamical systems using measurement data. Termed stochastic flow map learning (sFML), the new framework is an extension of flow map learning (FML) that was developed for learning deterministic dynamical systems. For learning stochastic systems, we define a stochastic flow map that is a superposition of two sub-flow maps: a deterministic sub-map and a stochastic sub-map. The stochastic training data are used to construct the deterministic sub-map first, followed by the stochastic sub-map. The deterministic sub-map takes the form of residual network (ResNet), similar to the work of FML for deterministic systems. For the stochastic sub-map, we employ a generative model, particularly generative adversarial networks (GANs) in this paper. The final constructed stochastic flow map then defines a stochastic evolution model that is a weak approximation, in term of distribution, of the unknown stochastic system. A comprehensive set of numerical examples are presented to demonstrate the flexibility and effectiveness of the proposed sFML method for various types of stochastic systems.

==> ProbEns.tex <==


\subsection{Probabilistic Ensemble Average}
\label{sec:ens}
The training of DNN involves inherent randomness because of stochastic optimization, thus resulting in predicting results with high variance. This uncertainty is also observed for GANs in our experiments. We emphasize that the unstable output accuracy is especially intractable in this case due to the involvement of random numbers. The ensemble average learning is a technique designed for decreasing the variance and improve the reliability of DNN models, see for example \cite{churchill2022robust,yang2020physics}. In this section, we propose an analogue of ensemble average technique under the context of probabilistic modeling. Our technique can be used in wider class of stochastic computing methods.

Let $\Gt_{\Delta}^{(i)}(\mathbf{x}_t)$, $i=1,2,...,M$ be $M$ models trained using aforementioned method. We then propose ensemble generator $\Gt^{(A)}(\mathbf{x}_t)$ as the following:
\begin{equation*}
    \Gt_{\Delta}^{(A)}(\mathbf{x}_t) = \Gt_{\Delta}^{(k)}(\mathbf{x}_t),~~~ k\sim \mathcal{U}(M),
\end{equation*}
where $\mathcal{U}(M)$ denotes the discrete uniform distribution among integers $1$ to $M$. Then we immediately have the following property:
\begin{proposition}
    Given $\mathbf{x}\in\mathbb{R}^d$ and measurable function $g: \mathbb{R}^d \mapsto \mathbb{R}^g$, $g\geq 1$, then the following averaging result holds for any measurable set $E$:
    \begin{equation}
        \mathbb{P}\left(g(\Gt_{\Delta}^{(A)}(\mathbf{x})) \in E\right) = \frac{1}{M} \sum_{i=1}^M \mathbb{P}\left(g(\Gt_{\Delta}^{(i)}(\mathbf{x})) \in E \right).
    \end{equation}
\end{proposition}
The above result shows the ensemble generator $\Gt_{\Delta}^{(A)}(\mathbf{x}_t)$ serves as an average of multiple models in a probabilistic sense. With this property, we found the ensemble generator consistently outperforms any of the averaged generators in estimating quantities we are interested in. For example, we consider the conditional mean $\D_\Delta (\mathbf{x})$ as defined in \eqref{equ:condmean}. Through direct computation, we also obtain the following averaging result:
\begin{equation}
    \begin{split}
        \D^{(A)}_\Delta\left(\mathbf{x}\right) & = \frac{1}{M}\sum_{i=1}^{M}\D^{(i)}_\Delta\left(\mathbf{x}\right),
    \end{split}
\end{equation}
where $\D^{(i)}_\Delta(\mathbf{x}) = \mathbb{E}(\Gt_\Delta^{(i)}(\mathbf{x}))$, $\D^{(A)}_\Delta(\mathbf{x}) = \mathbb{E}(\Gt_\Delta^{(A)}(\mathbf{x}))$. As a result,  the ensemble generator can estimate the conditional mean function $\D_\Delta (\mathbf{x})$ with lower variance. At each time point, we take this ensemble model to generate the predictions, it can be shown that the estimation is improved especially in the long time. Similar conclusion could be obtained for other quantities, such as the conditional variance function.

%To see the impact of randomness from optimization algorithms, we let $\boldsymbol{\mathcal{G}}_{\Delta}^{(i)}(\mathbf{x}_t)$ have trained parameter set $\Theta^{(i)}=(\Theta_{\boldsymbol{\mathcal{S}}})^{(i)}$. We further assume $\Theta^{(i)}$ are identical distributed mutually statistical independent (i.i.d.) with respect to the probability space of parameter space and denote:
%\begin{equation}
%    \Theta^{(i)} \stackrel{i.i.d.}{\sim} d_{\Theta}.
%\end{equation}
%For simplicity of notations, we denote $\mathbf{E}^{(i)}_\Delta\left(\mathbf{x}\right):=\mathbf{\widehat{E}}_\Delta\left(\mathbf{x},\Theta^{(i)}\right)$. Then the conditional expectation $\mathbf{E}^{(i)}_\Delta\left(\mathbf{x}\right)$ follow the push forward measure written as:
%\begin{equation}
%   \mathbf{E}^{(i)}_\Delta\left(\mathbf{x}\right)  \stackrel{i.i.d.}{\sim} \#_{\mathbf{\widehat{E}}_\Delta\left(\mathbf{x},\bullet\right)} d_{\Theta},~~i=1,2,...,M.
%\end{equation}
%Let
%\begin{equation}
%    \mathbb{E}_\Theta\left(\mathbf{\widehat{E}}_\Delta\left(\mathbf{x},\Theta\right)\right) = \mathbf{\widehat{E}}_\Delta(\mathbf{x}),~~\text{Cov}_\Theta\left(\mathbf{\widehat{E}}_\Delta\left(\mathbf{x},\Theta\right)\right) = \mathbf{\Sigma}_{\mathbf{\widehat{E}}_\Delta}(\mathbf{x}),
%\end{equation}
%Then the following Central Limit Theorem holds:
%\begin{proposition}
%    Given the above assumptions and condition $\mathbf{x}$, let $\mathbf{E}^{(A)}_\Delta\left(\mathbf{x}\right)$ be the conditional mean function of ensemble generator $\boldsymbol{\mathcal{G}}_{\Delta}^{(A)}(\mathbf{x})$. Then the following asymptotic result holds:
%    \begin{equation}
%        \sqrt{M}\left(\mathbf{E}^{(A)}_\Delta\left(\mathbf{x}\right)-\mathbf{\widehat{E}}_\Delta(\mathbf{x})\right) \stackrel{d}{\longrightarrow} \mathcal{N}\left(\mathbf{0},\mathbf{\Sigma}_{\mathbf{\widehat{E}}_\Delta}(\mathbf{x})\right),
%    \end{equation}
%\end{proposition}
%which shows the ensemble average generator $\boldsymbol{\mathcal{G}}_{\Delta}^{(A)}(\mathbf{x})$ is more efficient than any of averaged generators $\boldsymbol{\mathcal{G}}_{\Delta}^{(i)}(\mathbf{x})$ for estimated the conditional mean $\mathbf{E}_\Delta(\mathbf{x})$. These results will also be demonstrated in the numerical results of Section \ref{sec:numerical}.
